Maximum Entropy Based Significance of Itemsets

We consider the problem of defining the significance of an itemset. We say that the itemset is significant if we are surprised by its frequency when compared to the frequencies of its sub-itemsets. In other words, we estimate the frequency of the itemset from the frequencies of its sub-itemsets and compute the deviation between the real value and the estimate. For the estimation we use Maximum Entropy and for measuring the deviation we use Kullback-Leibler divergence. A major advantage compared to the previous methods is that we are able to use richer models whereas the previous approaches only measure the deviation from the independence model. We show that our measure of significance goes to zero for derivable itemsets and that we can use the rank as a statistical test. Our empirical results demonstrate that for our real datasets the independence assumption is too strong but applying more flexible models leads to good results.

==> motivation.tex <==
\section{Motivating Example}
\label{sec:motivation}
Consider the following 4 datasets, each having $8$ rows and $3$ attributes $a_1$, $a_2$, and $a_3$:
\[
D_1 = \set{\begin{array}{l}
\pr{0, 0, 0},
\pr{0, 0, 1},
\pr{0, 1, 0},
\pr{0, 1, 1}, \\
\pr{1, 0, 0},
\pr{1, 0, 1},
\pr{1, 1, 0},
\pr{1, 1, 1}
\end{array}},
\]
\[
D_2 = \set{\begin{array}{l}
\pr{0, 0, 0},
\pr{0, 0, 0},
\pr{0, 1, 1},
\pr{0, 1, 1}, \\
\pr{1, 0, 1},
\pr{1, 0, 1},
\pr{1, 1, 0},
\pr{1, 1, 0},
\end{array}},
\]
\[
D_3 = \set{\begin{array}{l}
\pr{0, 0, 1},
\pr{0, 0, 1},
\pr{0, 1, 0},
\pr{0, 1, 0}, \\
\pr{1, 0, 0},
\pr{1, 0, 0},
\pr{1, 1, 1},
\pr{1, 1, 1}
\end{array}},
\]
\[
D_4 = \set{\begin{array}{l}
\pr{0, 0, 1},
\pr{0, 0, 1},
\pr{0, 0, 1},
\pr{0, 0, 1}, \\
\pr{1, 1, 0},
\pr{1, 1, 0},
\pr{1, 1, 0},
\pr{1, 1, 0}.
\end{array}}.
\]

The frequencies for all itemsets of these datasets are given in Table~\ref{tab:exfreq}.

\begin{table}[htb!]
\center
\begin{tabular}{rrrrrrrrr}
\toprule
Data & $a_1$ & $a_2$ & $a_3$ & $a_1a_2$ & $a_1a_3$ & $a_2a_3$ & $a_1a_2a_3$ \\
\midrule
$D_1$ & $1/2$ & $1/2$ & $1/2$ & $1/4$ & $1/4$ & $1/4$ & $1/8$ \\
$D_2$ & $1/2$ & $1/2$ & $1/2$ & $1/4$ & $1/4$ & $1/4$ & $0$ \\
$D_3$ & $1/2$ & $1/2$ & $1/2$ & $1/4$ & $1/4$ & $1/4$ & $1/4$ \\
$D_4$ & $1/2$ & $1/2$ & $1/2$ & $1/2$ & $0$ & $0$ & $0$ \\
\bottomrule
\end{tabular}
\caption{Frequencies of itemsets for the toy datasets $D_1$--$D_4$.}
\label{tab:exfreq}
\end{table}

We ask ourselves: which itemsets given in Table~\ref{tab:exfreq} are
interesting? One way of measuring this is to compare the frequency of an
itemset to an estimation obtained from the independence model. In other words,
the more the frequency deviates from the independence assumption the more
interesting it is. The independence model predicts frequency $1/4$ for itemsets
$a_1a_2$, $a_1a_3$, and $a_2a_3$ and frequency $1/8$ for an itemset
$a_1a_2a_3$. Based on this measure, the itemset $a_1a_2a_3$ in the datasets
$D_2$, $D_3$ and $D_4$ is interesting and also the itemsets $a_1a_2$, $a_2a_3$,
and $a_1a_3$ in $D_4$ are interesting. Note that only the itemsets $a_1a_2$ in
$D_4$ and $a_1a_2a_3$ in $D_3$ are frequent.

In our scenario, the independence model predicts itemset frequencies from the
frequencies of $a_1$, $a_2$, and $a_3$. Let us assume that in addition we know
the frequencies of $a_1a_2$, $a_2a_3$, and $a_1a_3$ and we try to predict the
itemset $a_1a_2a_3$. For the datasets $D_1$--$D_3$ we see no reason for
changing the prediction $1/8$ for the frequency of $a_1a_2a_3$, because in
these datasets the itemsets $a_1a_2$, $a_1a_3$, and $a_2a_3$ agree with the
independence model. Thus $a_1a_2a_3$ remains interesting in $D_2$ and $D_3$.
However, in $D_4$ we can deduce from $a_1a_3$ (or from $a_2a_3$) that
$a_1a_2a_3$ must be $0$. Thus under this assumption $a_1a_2a_3$ is no longer
interesting in $D_4$.

We wish to emphasize two points with this example: First, frequency does not
necessarily mean significance. We may find certain infrequent itemsets
interesting and some frequent itemset not interesting. Second, the independence
model may be inadequate.  We may find that itemsets become less interesting if
we apply richer models.

